Sidebar: Scratchpad Based Communication Between CPUs and Accelerators

Hardware accelerators for neural networks have shown great promise for both performance and power. These accelerators are at their most efficient when optimized for a fixed functionality. But this inflexibility limits the longevity of the hardware itself as the underlying neural network algorithms and structures undergo improvements and changes. We propose and evaluate a flexible design paradigm for accelerators with a close coordination with host processors. The relatively static matrix operations are implemented in specialized accelerators while fast-evolving functions, such as activations, are computed on the host processor. This architecture is enabled by a low latency shared buffer we call Sidebar. Sidebar memory is shared between the accelerator and host, exists outside of program address space and holds intermediate data only. We show that a generalised DMA dependent flexible accelerator design performs poorly in both perf and energy as compared to an equivalent fixed function accelerator. Sidebar based accelerator design achieves near identical performance and energy to equivalent fixed function accelerator while still providing all the flexibility of computing activations on the host processor.

==> progress.tex <==
\section{Progress}
The first main progress we made was refining and clarifying our project goals and statement. This was mostly based on the feedback we received from the initial project presentation and Professor Adve's inputs and feedback. The exact changes are already addressed in this document but can be summarized as below:
\begin{enumerate}
    \item Focus on the aspect of the project where activations are computed by the CPU.
    \item Complete removal of analysis of using the scratchpad for initial data movement to the accelerator, replacing DMA.
    \item Scrachpad is now only used to enable fine-grained cooperation with CPU.
\end{enumerate}

Second, we decided the evaluation example. We will use AlexNet \cite{alexnet} training as the evaluation example. This network uses ReLU activations (and in fact introduced them). We will evaluate computing ReLU in a variety of ways, but we will also evaluate the model with other activation functions. We are unconcerned with the accuracy of the models, directing our analysis entirely on the latency of computing a forward pass. For our evaluation we will compare:
\begin{enumerate}
    \item Fully ASIC implementation of AlexNet, with alternative activations:
    \begin{enumerate}
        \item sigmoid
        \item tanh (hyperbolic tangent)
        \item Leaky ReLU
        \item Noisy ReLU
    \end{enumerate}
    \item A standard interface use of AlexNet where the activation is done on the CPU, and data is transferred by DMA.
    \item Our proposed implementation, where the scratchpad is used to accelerate the movement of data back for the CPU to perform the activations.
\end{enumerate}

Third, we have been trying to set up gem5-Aladdin to set up the evaluation for this project. At the moment we are still trying to get a basic setup working. While we have a gem5 setup running, the Aladdin dependencies are proving challenging on our system. If we are unable to resolve these soon we plan on looking into alternative options. The first option is a Docker image created by the gem5-Aladdin authors. The image is rather old, but we can try to use it as a starting point. The second option would be to consult other groups also looking to utilize gem5-Aladdin in their projects. 
